Tight analyses of first-order methods with error feedback

Communication between agents often constitutes a major computational bottleneck in distributed learning. One of the most common mitigation strategies is to compress the information exchanged, thereby reducing communication overhead. To counteract the degradation in convergence associated with compressed communication, error feedback schemes -- most notably $\mathrm{EF}$ and $\mathrm{EF}^{21}$ -- were introduced. In this work, we provide a tight analysis of both of these methods. Specifically, we find the Lyapunov function that yields the best possible convergence rate for each method -- with matching lower bounds. This principled approach yields sharp performance guarantees and enables a rigorous, apples-to-apples comparison between $\mathrm{EF}$, $\mathrm{EF}^{21}$, and compressed gradient descent. Our analysis is carried out in the simplified single-agent setting, which allows for clean theoretical insights and fair comparison of the underlying mechanisms.

==> certified.tex <==
% certified.tex — \certifiedblock (default: BRACE) and \certifiedbox (always BOX)
\ProvidesFile{certified.tex}[2025/10/17 Certified block (brace+box)]
\usepackage{stmaryrd}
\usepackage{fontawesome5}

% Core
\RequirePackage{xparse}
\RequirePackage{etoolbox}
\RequirePackage{graphicx}
\RequirePackage{pgfkeys}
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathreplacing,calc}

% tcolorbox + hyperlinks/footnotes (load only if needed)
\makeatletter
\@ifpackageloaded{tcolorbox}{}{\RequirePackage{tcolorbox}}
\tcbuselibrary{skins,breakable}
\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\@ifpackageloaded{footnotehyper}{}{\RequirePackage{footnotehyper}} % after hyperref
\makeatother
\makesavenoteenv{tcolorbox}  % footnotes inside the box go to the page bottom

% Also search for icons where this file lives (if currfile is available)
\IfFileExists{currfile.sty}{%
  \RequirePackage{currfile}
  \makeatletter \edef\certblockdir{\currfiledir} \makeatother
  \graphicspath{{\certblockdir}{./}}
}{}

% Tunables for brace style
\newlength\CertifiedBraceGap    \setlength\CertifiedBraceGap{0.9em}
\newlength\CertifiedBraceRise   \setlength\CertifiedBraceRise{4pt}
\newcommand\CertifiedBraceWidth{1pt}
\newcommand\CertifiedBraceAmp{5pt}
\newcommand\CertifiedBraceColor{blue}

% Keys: cas=<url>, pep=<url>, style=brace|box (default=brace)
\pgfkeys{
  /certblock/.is family,
  /certblock/.cd,
  cas/.initial=,
  pep/.initial=,
  style/.initial=brace,      % default = BRACE
  % aliases so user can write simply [box] or [brace]
  box/.code   = \pgfkeysalso{/certblock/style=box},
  brace/.code = \pgfkeysalso{/certblock/style=brace},
  badgeheight/.initial=1.0em,
}

% Storage
\newcommand*\certblockcas{}
\newcommand*\certblockpep{}
\newcommand*\certblockstyle{brace}

% Parse helper (robust)
\newcommand*\certblockParse[1]{%
\pgfkeys{/certblock/.cd, cas=, pep=, style=brace, badgeheight=1.0em}%
  \pgfkeys{/certblock/.cd, #1}%
  \pgfkeysgetvalue{/certblock/cas}{\certblockcas}%
  \pgfkeysgetvalue{/certblock/pep}{\certblockpep}%
  \pgfkeysgetvalue{/certblock/style}{\certblockstyle}%
}

\newcommand*\certcasiconfile{CAS.pdf}
\newcommand*\certcasbadgefile{CAS_inv.pdf}


% Icons (small; used near brace or in box title)
\newcommand*\certblockicons{%
  \begingroup\setlength{\fboxsep}{0pt}%
  \def\out{}%
  \ifdefempty{\certblockcas}{}{%
    \edef\out{\out\noexpand\href{\certblockcas}{\noexpand\raisebox{-0.2ex}{\noexpand \includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{\certcasiconfile}}}}%
  }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\out}{}{\edef\out{\out\noexpand\hspace{0.4em}}}%
    \edef\out{\out\noexpand\href{\certblockpep}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{PEP.pdf}}}}%
  }%
  \out
  \endgroup
}

% Badge text (used ONLY when style=box AND no icons)
\newcommand*\certblockbadge{%
  \begingroup
  \def\result{external sources}%
  \ifdefempty{\certblockcas}{}{ \def\result{CAS} }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\certblockcas}{\def\result{PEP}}{\def\result{CAS \& PEP}}%
  }%
  \result
  \endgroup
}

% For general icons, \certcasiconfile may be changed; the far-right badge uses
% \certcasbadgefile (CAS_inv.pdf) to explore alternate palette
% \def\certcasiconfile{CAS_green.pdf}

% ----- Theme knobs (safe to \renewcommand in main.tex) -----
% Box and title colors (defaults match current palette)
\newcommand*\CertifiedFrameColor{green!75!black}
\newcommand*\CertifiedBackColor{green!12}
% Use an explicit sRGB hex for header background to avoid CMYK→RGB variations
\definecolor{CertifiedHeaderGreen}{HTML}{258E58}
\newcommand*\CertifiedTitleBack{CertifiedHeaderGreen}
\newcommand*\CertifiedTitleTextColor{white}
% Small right-side badge (chip) colors
\newcommand*\CertifiedBadgeFill{none}
\newcommand*\CertifiedBadgeDraw{none}
\newcommand*\CertifiedBadgeTextColor{black}
% Badge text sizing and padding
\newcommand*\CertifiedBadgeFontSize{\scriptsize}
\newcommand*\CertifiedBadgeInnerX{4pt}
\newcommand*\CertifiedBadgeInnerY{2pt}

% Optional key to override title text color per-call
\pgfkeys{ /certblock/.cd, titletextcolor/.initial=} % blank means use macro default

% Geometry & radii (safe to override)
\newcommand*\CertifiedArc{6pt} % used for main box and chip
\newcommand*\CertifiedRightArc{2pt} % smaller arc on chip's right corners
% Chip anchor offset relative to interior corner (prefer 0pt to align exactly)
\newcommand*\CertifiedChipOffsetX{0pt}
\newcommand*\CertifiedChipOffsetY{0pt}
% Gap between chip text and right-side badge
\newcommand*\CertifiedBadgeOffsetX{4pt}
\newcommand*\CertifiedBadgeOffsetY{0pt}
% Inset of the badge from the right interior edge of the box
\newcommand*\CertifiedBadgeRightInset{0pt}

% ----- Renderers -----
% put this near your other \newcommand's, BEFORE \certBadgeContent
\newcommand{\certExtIcon}{%
  \raisebox{0.15ex}{\scalebox{0.85}{\faIcon{external-link-alt}}}%
}
\newcommand{\certBadgeContent}{%
  {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize
   CAS\hspace{0.4em}\certExtIcon}%
}
\newcommand*\certblockRenderBox[1]{%
  % Decide title: icons inline if present; else text badge
  % Determine if we have icons (for the right-side badge)
  \newif\ifcertblockhasicons
  \certblockhasiconsfalse
  \ifdefempty{\certblockcas}{}{ \certblockhasiconstrue }%
  \ifdefempty{\certblockpep}{}{ \certblockhasiconstrue }%

  % Title text always present (keep text inside the chip)
  \edef\certblocktitletext{\noexpand\emph{Certified using WolframScript}}%

  % Resolve per-call title font color (fallback to macro default)
  \def\certblocktitlecolor{\CertifiedTitleTextColor}%
  % Avoid '@' in control sequence names (no \makeatletter needed)
  \pgfkeysgetvalue{/certblock/titletextcolor}{\certblocktitletextcolor}%
  \ifdefempty{\certblocktitletextcolor}{}{\edef\certblocktitlecolor{\certblocktitletextcolor}}%

  \begin{tcolorbox}[
    enhanced,
    arc=\CertifiedArc,
    width=\linewidth,
    boxrule=0pt, % remove main border
    colframe=\CertifiedFrameColor,
    colback=\CertifiedBackColor,
    left=6pt,right=6pt,top=16pt,bottom=6pt,
    overlay={%
      % Measure the chip area with an invisible node (for precise geometry)
      \node[inner xsep=6pt, inner ysep=2pt,
            anchor=north west, outer sep=0pt,
            opacity=0] (certchip)
        at ([xshift=\CertifiedChipOffsetX,yshift=\CertifiedChipOffsetY]interior.north west)
          {\certblocktitletext};
      % Base chip background with standard arc (top-left rounded)
      \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
        (certchip.north west) rectangle (certchip.south east);
      % Square off the lower-left corner of the chip to be flush with left edge
      \path[fill=\CertifiedTitleBack, draw=none]
        (certchip.south west) rectangle ++(\CertifiedArc,\CertifiedArc);
      % Replace the right corners with a smaller arc by overdrawing only the
      % right half using a second rounded rectangle with a smaller radius.
      \begin{scope}
        \clip (certchip.center |- certchip.north east)
              rectangle
              (certchip.south east);
        \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
          (certchip.north west) rectangle (certchip.south east);
      \end{scope}
      % Foreground text (white), placed after background painting
      \node[anchor=north west, outer sep=0pt,
            text=\certblocktitlecolor, font=\itshape]
        at (certchip.north west) {\certblocktitletext};
      % Add the right-side badge aligned with the chip, anchored to the
      % right interior edge of the box with optional inset. Use text box
      % "CAS" (Helvetica, selectable) if CAS link is provided; otherwise
      % fall back to icon variant.
      \ifcertblockhasicons
        \ifdefempty{\certblockcas}{%
          \node[anchor=east, outer sep=0pt]
            at ([xshift=-\CertifiedBadgeRightInset, yshift=\CertifiedBadgeOffsetY]interior.north east |- certchip.east)
              {\begingroup\color{\CertifiedBadgeTextColor}\certblockiconsbadge\endgroup};
        }{%
          % Build a text-based CAS pill with the SAME vertical extent as the
          % left header chip, so the corner radius matches exactly.
          % Right edge is flush with the box interior (minus any inset).
          \begin{scope}
            % Key reference points
            \coordinate (badgeTR) at ([xshift=-\CertifiedBadgeRightInset]interior.north east);
            \coordinate (badgeBR) at ([xshift=-\CertifiedBadgeRightInset]interior.south east |- certchip.south);
            % Measure the CAS text at the correct baseline and padding
            \node[anchor=base east, inner sep=0pt, outer sep=0pt, opacity=0] (castxt)
              at ([xshift=-\CertifiedBadgeRightInset-\CertifiedBadgeInnerX]interior.north east |- certchip.base east)
              {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize \certBadgeContent};
            % Compute left edge from measured width + padding
            \coordinate (badgeLX) at ([xshift=-\CertifiedBadgeInnerX]castxt.west);
            \coordinate (badgeTL) at (badgeLX |- certchip.north);
            \coordinate (badgeBL) at (badgeLX |- certchip.south);
            % Base background with LARGE radius everywhere
            \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
              (badgeTL) rectangle (badgeBR);
            % Overpaint LEFT side with SMALL radius to adjust left corners only
            \begin{scope}
              \clip (badgeTL) rectangle (castxt.center |- badgeBR);
              \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
                (badgeTL) rectangle (badgeBR);
            \end{scope}
            % Square the bottom-right to remove rounding
            \path[fill=\CertifiedTitleBack, draw=none]
              (badgeBR) rectangle ++(-\CertifiedArc,\CertifiedArc);
            % Foreground (clickable) text in Helvetica, white
            \node[anchor=base east, inner sep=0pt, outer sep=0pt]
              at (castxt.base east)
              {\href{\certblockcas}{\textcolor{\CertifiedTitleTextColor}{\fontfamily{phv}\selectfont\CertifiedBadgeFontSize \certBadgeContent}}};
          \end{scope}
        }%
      \fi
    },
  ]#1\end{tcolorbox}%
}

\newcommand*\certblockRenderBrace[1]{%
  \begin{tcolorbox}[
    enhanced, blanker,
    left=0pt, right=0pt, top=0pt, bottom=0pt,
    boxsep=0pt, width=\linewidth,
    before upper=\setlength{\parindent}{0pt},
    overlay={%
      % Left-facing brace drawn to the LEFT of the text block
      \draw[
        draw=\CertifiedBraceColor, line width=\CertifiedBraceWidth,
        decorate, decoration={brace,mirror,amplitude=\CertifiedBraceAmp}
      ]
        ([xshift=-\CertifiedBraceGap, yshift=\CertifiedBraceRise]frame.north west)
          --
        ([xshift=-\CertifiedBraceGap, yshift=-\CertifiedBraceRise]frame.south west)
        % Optional icons to the LEFT of the brace, centered vertically
        node[midway, anchor=east, xshift=-0.4em]{\certblockicons};
    }
  ]#1\end{tcolorbox}%
}

% ----- Public commands -----
% \certifiedbox[cas=<url>, pep=<url>]{<content>}  -> ALWAYS BOX
\NewDocumentCommand{\certifiedbox}{ O{} +m }{%
  \certblockParse{#1}%
  \certblockRenderBox{#2}%
}

% \certifiedblock[style=brace|box, cas=<url>, pep=<url>]{<content>}  -> DEFAULT BRACE
\NewDocumentCommand{\certifiedblock}{ O{} +m }{%
  \certblockParse{#1}%
  \ifdefstrequal{\certblockstyle}{box}{%
    \certblockRenderBox{#2}%
  }{%
    \certblockRenderBrace{#2}%
  }%
}

% ---- Standalone CAS badge (Helvetica, white text) ---------------------------
% Shape: left corners = \CertifiedRightArc, top-right = \CertifiedArc,
%        bottom-right = square (no rounding). Background = \CertifiedTitleBack.
% Usage: \certcasbox  (inline box containing "CAS")
\newcommand*\certlabelbox[1]{%
  \tikz[baseline=(txt.base)]{
    % Measure content with padding
    \node[inner xsep=\CertifiedBadgeInnerX, inner ysep=\CertifiedBadgeInnerY, outer sep=0pt,
          anchor=base west, opacity=0] (txt) {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize #1};
    % Base background with small-radius corners everywhere
    \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
      (txt.north west) rectangle (txt.south east);
    % Overpaint right half with larger radius for the top-right corner
    \begin{scope}
      \clip (txt.center |- txt.north east) rectangle (txt.south east);
      \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
        (txt.north west) rectangle (txt.south east);
    \end{scope}
    % Flatten bottom-right (square off)
    \path[fill=\CertifiedTitleBack, draw=none]
      (txt.south east) rectangle ++(-\CertifiedArc,\CertifiedArc);
    % Foreground text
    \node[anchor=base west, outer sep=0pt, text=\CertifiedTitleTextColor]
      at (txt.base west) {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize #1};
  }%
}

\newcommand*\certcasbox{\certlabelbox{CAS}}

% ===================== Add-on: certified (keeps certifiedblock intact) =====================

% Safe package hooks
\makeatletter
\@ifpackageloaded{thmtools}{}{%
  \RequirePackage{thmtools}
  \RequirePackage{thm-restate}
}
\@ifpackageloaded{xparse}{}{\RequirePackage{xparse}}
\@ifpackageloaded{pgfkeys}{}{\RequirePackage{pgfkeys}}
\@ifpackageloaded{etoolbox}{}{\RequirePackage{etoolbox}}
\@ifpackageloaded{graphicx}{}{\RequirePackage{graphicx}}
\makeatother

% ---- Link helper without '@' in the name (robust to load order)
\providecommand\certhref[2]{#2}% default: no link if hyperref isn't loaded yet
\makeatletter
\@ifpackageloaded{hyperref}{%
  \renewcommand\certhref[2]{\href{#1}{#2}}%
}{%
  % If hyperref loads later, upgrade certhref then:
  \AtBeginDocument{%
    \@ifpackageloaded{hyperref}{\renewcommand\certhref[2]{\href{#1}{#2}}}{}%
  }%
}
% Backward-compat for any prior snippet that used \cert@href:
\providecommand\cert@href[2]{\certhref{#1}{#2}}
\makeatother

% ======== Robust keys + parser for theorem badges (NO expl3 / NO \zap@space) ========
\makeatletter

% Booleans indicating whether to actually show each badge
\newif\ifcertthm@cas
\newif\ifcertthm@pep

% Storage (safe if already defined)
\providecommand*\certthmcas{}
\providecommand*\certthmpep{}
\providecommand*\certthmbadgeheightraw{1.0em}
\@ifundefined{certthmbadgeheight}{\newlength\certthmbadgeheight}{}

% Key family with robust emptiness checks (PGF's \pgfutil@ifempty)
\pgfkeys{/certthm/.is family, /certthm,
  cas/.code={
    \pgfutil@ifempty{#1}{%
      \certthm@casfalse \def\certthmcas{}%
    }{%
      \certthm@castrue  \def\certthmcas{#1}%
    }%
  },
  pep/.code={
    \pgfutil@ifempty{#1}{%
      \certthm@pepfalse \def\certthmpep{}%
    }{%
      \certthm@peptrue  \def\certthmpep{#1}%
    }%
  },
  badgeheight/.code={
    \pgfutil@ifempty{#1}{%
      \def\certthmbadgeheightraw{1.0em}% default if blank or omitted
    }{%
      \def\certthmbadgeheightraw{#1}%
    }%
  },
}

% Parse once per environment: reset flags, apply keys, commit length
\providecommand*\certthmParse{}%
\renewcommand*\certthmParse[1]{%
  \certthm@casfalse \certthm@pepfalse
  \def\certthmcas{}%
  \def\certthmpep{}%
  \def\certthmbadgeheightraw{1.0em}%
  \pgfkeys{/certthm/.cd, #1}%
  \setlength{\certthmbadgeheight}{\certthmbadgeheightraw}%
}

% ---- Vertically center a badge image to the line's "Theorem X" height
\newcommand{\certcenterimg}[1]{%
  \raisebox{.5\dimexpr\ht\strutbox - \dp\strutbox - \certthmbadgeheight\relax}%
           [\ht\strutbox][\dp\strutbox]{%
             \includegraphics[height=\certthmbadgeheight]{#1}}%
}

% ---- Assemble badges (CAS.pdf / PEP.pdf). Clickable if hyperref is present.
\makeatletter
\providecommand*\certthmicons{}% ensure the macro exists before renewing
\renewcommand*\certthmicons{%
  \begingroup
    \ifcertthm@cas
      \certhref{\certthmcas}{\certcenterimg{CAS.pdf}}%
    \fi
    \ifcertthm@pep
      \ifcertthm@cas\hspace{0.4em}\fi
      \certhref{\certthmpep}{\certcenterimg{PEP.pdf}}%
    \fi
    \endgroup
}

% Icons variant for the far-right header badge (uses CAS_inv.pdf)
\newcommand*\certblockiconsbadge{%
  \begingroup\setlength{\fboxsep}{0pt}%
  \def\out{}%
  \ifdefempty{\certblockcas}{}{%
    \edef\out{\out\noexpand\href{\certblockcas}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{\certcasbadgefile}}}}%
  }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\out}{}{\edef\out{\out\noexpand\hspace{0.4em}}}%
    \edef\out{\out\noexpand\href{\certblockpep}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{PEP.pdf}}}}%
  }%
  \out
  \endgroup
}
\makeatother
% ---- Wrapper environment: certified
% Capture the body (+b) and emit a full restatable block so the collector
% sees \end{restatable}. The theorem BODY always starts on a new line.
%
% Usage:
%   \begin{certified}[cas=<url>, pep=<url>, badgeheight=<len>]{theorem}{<cmd>}[<header>]
%     <theorem body>
%   \end{certified}
% Note: <cmd> must be a bare name (no leading backslash), e.g., {myThm}.
\NewDocumentEnvironment{certified}{ O{} m m O{} +b }{%
  \certthmParse{#1}%
  \begin{restatable}[#4]{#2}{#3}%
    \certthmicons\mbox{}%
    \par\vspace{-\parskip}%
    \setlength{\parindent}{0pt}\noindent\ignorespaces
    
    #5%
  \end{restatable}%
}{}

% =================== End add-on: certified (certifiedblock left unchanged) ===================

% --- Certificate notice (simple, non-clickable) -----------------
\RequirePackage{graphicx} % very common; safe if already loaded

% Tiny knobs you can tweak via \renewcommand in your main file:
\newcommand{\certnoticeheight}{2.0em} % badge height
\newcommand{\certnoticesep}{2em}      % horizontal gap between badges
\newcommand{\certnoticevspace}{-2em}  % vertical space before the notice

\newcommand{\makecertificatenotice}{%
  \vspace*{\certnoticevspace}%
  \begin{center}
    \emph{Proof certificates are annotated using\footnote{We generate certificates of validity using a Computer Algebra System (CAS, via WolframScript) and Performance Estimation Problems (PEP). CAS annotations mark partial verification of proof identities, whereas PEP annotations indicate full verification of the statement. Each annotation links to the corresponding file in our GitHub repository}}%
    \par
    \includegraphics[height=\certnoticeheight]{CAS.pdf}\hspace{\certnoticesep}%
    \includegraphics[height=\certnoticeheight]{PEP.pdf}%
  \end{center}%
}
% ---------------------------------------------------------------


\newtcolorbox{caspara}[1][]{%
  breakable,
  enhanced,
  colback=\CertifiedBackColor,
  colframe=ForestGreen,
  arc=0pt,
  outer arc=0pt,
  title=Remark: proof certificates,
  fonttitle=\bfseries\sffamily,
  colbacktitle=ForestGreen,
  attach boxed title to top left={},
  boxed title style={
    enhanced,
    skin=enhancedfirst jigsaw,
    arc=3pt,
    bottom=0pt,
    interior style={fill=ForestGreen}
  }
}
\makesavenoteenv{caspara}

